IMB-NAS: Neural Architecture Search for Imbalanced Datasets

Class imbalance is a ubiquitous phenomenon occurring in real world data distributions. To overcome its detrimental effect on training accurate classifiers, existing work follows three major directions: class re-balancing, information transfer, and representation learning. In this paper, we propose a new and complementary direction for improving performance on long tailed datasets - optimizing the backbone architecture through neural architecture search (NAS). We find that an architecture's accuracy obtained on a balanced dataset is not indicative of good performance on imbalanced ones. This poses the need for a full NAS run on long tailed datasets which can quickly become prohibitively compute intensive. To alleviate this compute burden, we aim to efficiently adapt a NAS super-network from a balanced source dataset to an imbalanced target one. Among several adaptation strategies, we find that the most effective one is to retrain the linear classification head with reweighted loss, while freezing the backbone NAS super-network trained on a balanced source dataset. We perform extensive experiments on multiple datasets and provide concrete insights to optimize architectures for long tailed datasets.

==> sections/methodolody-v1.tex <==
\section{Methodology}
\subsection{Problem Setup}
\textbf{Notation:} Assume $\mathcal{D} = \{x_1,y_i\}$ denotes the training dataset of images where $y_i$ is the label for image $x_i$. Let $n_j$ specify the number of training images in class $j$. After sorting the classes by cardinality in decreasing order, the long tail assumption specifies that if $i<j$, then $n_i \geq n_j$ and $n_1>>n_C$. We use $\phi$ to denote a deep neural network that is composed of a backbone $\phi(a,w_a)$ with architecture $a$, weights $w_a$ and a linear classifier $\phi(w_c)$. The model $\phi$ is trained using a training loss and loss re-weighting strategy. I this work we use the cross entropy loss (denoted as CE) and the effective re-weighting strategy that reweights samples from class $j$ with $\frac{1-\beta}{1-\beta^{n_j}}$ where $\beta$ is a hyperparameter. Following previous works, the re-weighting strategy is applied after a delay of few training epochs which is denoted using the shorthand DRW. 
%The overall training procedure with CE loss and DRW schedule is denoted by $\mathcal{T}_{CE+DRW}$.

\textbf{Formulation:}
Given a search space of architectures $\mathcal{A}$, a dataset $\mathcal{D}$, and a training procedure $\mathcal{T}$ we denote a rank ordering by $\mathcal{R}(\mathcal{T}(A, D))$ that ranks architectures $\{a_i\}\in A$ such that $a_i<a_j$ if $a_i$ achieves lower validation accuracy than $a_j$. 
%
Our setup assumes two datasets: a source dataset $D_s$, a target dataset $D_t$ and associated trainind procedures $\mathcal{T}_s$, $\mathcal{T}_t$ that induce the architectural orderings $\mathcal{R}(\mathcal{T}_s(A,D_s))$ and $\mathcal{R}(\mathcal{T}_t(A,D_t))$.
%
The goal of this paper is to develop the most \textit{efficient} rank adjustment procedure $\mathcal{P}$ that can transform the source rank order to approximate the target rank order, or formally, $\mathcal{R}( \mathcal{P} (\mathcal{T}_{s}(A, D_s), D_t) \approx \mathcal{R}(\mathcal{T}_{t}(A, D_t))$.


\begin{figure}[!h]%
    \centering
    % \subfloat[\centering Cifar-10 to Cifar-10]{{\includegraphics[width=0.45\columnwidth]{Figures/Fig_1/c10_c10.png} }}%
    % \qquad
    % \subfloat[\centering Cifar-100 to Cifar-100]{{\includegraphics[width=0.45\columnwidth]{Figures/Fig_1/c100_c100.png} }}%
    % \qquad
    \subfloat[\centering Cifar-10 to Cifar-100]{{\includegraphics[width=0.45\columnwidth]{Figures/Fig_1/c10_c100.png} }}%
    % \qquad
    \subfloat[\centering Cifar-100 to Cifar-10]{{\includegraphics[width=0.45\columnwidth]{Figures/Fig_1/c100_c10.png} }}%
    \caption{Color range should be the same.}%
    \label{fig:example}%
\end{figure}


\subsection{Motivating study}

We study the impact of backbone architecture on imbalanced datasets using the following experiment.
%
We construct an architecture search space $A$ by sampling all 149 Mega Flops architectures from the NATS-bench search space.
%
Overall $A$ contains 135 architectures with exactly the same learning capacity (or Flops), but different architectural patterns (e.g. kernel sizes, layer connectivity).
%
The architectures in $A$ are trained on the source and target datasets $D_s, D_t$ using training strategies $\mathcal{T}_s, \mathcal{T}_t$.
%
Following this, the architecture rank orderings $\mathcal{R}_s(T_s(A,D_s))$, $\mathcal{R}_t(T_s(A,D_t))$ are determined and we measure the kendall tau rank correlation $\tau(\mathcal{R}_s,\mathcal{R}_t)$.
%
A high correlation means similar architectural rankings while a low correlation implies widely different rankings.

We consider two scenarios: (1) $D_s$ and $D_t$ are from the same dataset (e.g. cifar-100), but differ due to class imbalance; and (2) $D_s$ and $D_t$ are from different datasets (e.g. cifar-100), and also differ due to class imbalance (e.g. cifar-100 and cifar-10).
%
For training on class balanced datasets, $\mathcal{T}$ uses the cross entropy loss and is denoted by $\mathcal{T}_{CE}$. 
%
On the other hand, $\mathcal{T}$ for imbalance datasets uses cross entropy loss with delayed reweighting and is denoted by $\mathcal{T}_{CE+DRW}$.
%

The two scenario are outlined in Fig. XX which plots the rank-correlation between three versions of Cifar-100 and Cifar-10 (1x, 50x and 100x imbalance).
%
There are two major observations---First, the low correlation in the off-diagonal entries indicates that the architectural rankings widely differ on imbalanced versions of the same dataset.
%
This means the optimal architecture for a balanced dataset may not be the optimal one for imbalanced datasets.
%
Second, the high correlation in bottom left squares (i.e. between balanced $D_s, D_t$) indicates that the architectural rankings are transferable across fully class balanced datasets. 
%
This observation validates a key assumption of existing NAS methods: the optimal model on ImageNet (fully class balanced dataset) is also optimal for other class balanced datasets. 

\subsection{Revisiting NAS}
In this work, we focus on sampling based NAS methods that involve two steps. The first step involves training a super-network with backbone $\phi(a, w_a)$ and classifier $\phi(w_c)$ on a training dataset $D$ via the following minimization
\begin{equation}
    w^{*}_{a, \mathcal{D}}, w^{*}_{c,  \mathcal{D}} = \mathop{min}_{w_a,w_c} \mathop{\mathbb{E}}_{a \sim \mathcal{A}} \left( \mathcal{L}(\phi(w_c),\phi(a, w_a); \mathcal{D})   \right).
\end{equation}
Here the inner expectation is performed by sampling architectures $a$ from a search space $\mathcal{A}$ via uniform, or attentive sampling.

The second step involves searching the optimal architecture that maximizes validation accuracy via the following optimisation
\begin{equation}
    a^*_{\mathcal{D}} = \mathop{max}_{a \in \mathcal{A}} Acc \left( \phi(w_c),\phi(a, w_a); \mathcal{D})   \right).
\end{equation}
This maximization is typically implemented via evolutionary search or reinforcement learning.

\subsection{Rank adjustment procedures}

\rahul{Rank adjustment sounds incremental. Can change it to super-net adaptation procedure.}
\rahul{Can call P1/P2 as SuperAdapt}
Given source and target datasets $\mathcal{D}_s, \mathcal{D}_t$, we first train a super-network on $D_s$ by solving the following optimisation
\begin{equation}
\label{eq:p0_eqn}
    w^{*}_{a, \mathcal{D}_s}, w^{*}_{c,  \mathcal{D}_s} = \mathop{min}_{w_a,w_c} \mathop{\mathbb{E}}_{a \sim \mathcal{A}} \left( \mathcal{L}(\phi(w_c),\phi(a, w_a); \mathcal{D}_s)   \right).
\end{equation}
% Here the inner expectation is computed by sampling n architectures $a$ from a search space $\mathcal{A}$ via uniform, or attentive sampling.
Our goal then is to adapt the optimal super-net weights $w^{*}_{a, \mathcal{D}_s}, w^{*}_{c,  \mathcal{D}_s}$ found on $D_s$ to the target dataset $D_t$ which suffers from class imbalance. The most efficient adjustment procedure involves freezing the backbone, while adjusting only the linear classifier on $D_t$ by minimizing the re-weighted loss $\mathcal{L}_{RW}$
\begin{equation}
\label{eq:p1_eqn}
    w^{*}_{c,  \mathcal{D}_t} = \mathop{min}_{w_c} \mathop{\mathbb{E}}_{a \sim \mathcal{A}} \left( \mathcal{L}_{RW}(\phi(w_c),\phi(a, w^{*}_{a, \mathcal{D}_s}); \mathcal{D}_t)   \right).
\end{equation}
The resulting super-network contains backbone weights $w^{*}_{a, \mathcal{D}_s}$ trained on $\mathcal{D}_s$ and classifier weights $w^{*}_{c,  \mathcal{D}_s}$ trained on $\mathcal{D}_t$.  Solving the above optimisation is extremely efficient since most of the network is frozen while only the classifier is trained. On the other hand, one could also adjust the backbone by fine-tuning on the target dataset. This is achieved by minimizing the delayed re-weighted loss $\mathcal{L}_{DRW}$
\begin{equation}
\label{eq:p2_eqn}
    w^{**}_{a,  \mathcal{D}_t}, w^{*}_{c,  \mathcal{D}_t} = \mathop{min}_{w_a, w_c} \mathop{\mathbb{E}}_{a \sim \mathcal{A}} \left( \mathcal{L}_{DRW}(\phi(w_c),\phi(a, w^{*}_{a, \mathcal{D}_s}); \mathcal{D}_t)   \right).
\end{equation}
 Here, the double star on $w^{**}_{a,  \mathcal{D}_t}$ indicates the weights were obtained via fine-tuning $w^{*}_{a, \mathcal{D}_s}$ using one tenth of the original learning rate and one third the number of original training epochs. Also, recall that the delayed re-weighted loss $\mathcal{L}_{DRW}$ is nothing but the unweighted loss $\mathcal{L}$ in the first few epochs and the re-weighted loss $\mathcal{L}_{RW}$ subsequently. Note that our second adjustment procedure is more compute intensive since the backbone is also adjusted, but still much less intensive than running the full search on the target dataset.
 
Our final and most compute intensive procedure involves directly searching on the target dataset via $\mathcal{L}_{DRW}$. This is achieved via the following minimization 
 \begin{equation}
 \label{eq:p3_eqn}
    w^{*}_{a, \mathcal{D}_t}, w^{*}_{c,  \mathcal{D}_t} = \mathop{min}_{w_a,w_c} \mathop{\mathbb{E}}_{a \sim \mathcal{A}} \left( \mathcal{L}_{DRW}(\phi(w_c),\phi(a, w_a); \mathcal{D}_t)   \right).
\end{equation}
% \subsection{Measuring rank adjustment}
The three adjustment procedures and their associated compute costs are summarized in Table.XXXX.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{ccl}
\toprule
\textbf{Adj} & \textbf{Eq} & \multicolumn{1}{c}{\textbf{Description}}                              \\ \midrule
P0           &      (\ref{eq:p0_eqn})        & No adjustment. \\
P1           &      (\ref{eq:p1_eqn})        & Freeze backbone, retrain classifier on $\mathcal{D}_t$.                      \\
P2           &      (\ref{eq:p2_eqn})        & Finetune backbone and retrain classifier on $\mathcal{D}_t$      \\
P3           &      (\ref{eq:p3_eqn})        & Re-train backbone and classifier on $\mathcal{D}_t$.\\ \bottomrule
\end{tabular}
\end{table}
